LargeEA: Aligning Entities for Large-scale Knowledge Graphs

Entity alignment (EA) aims to find equivalent entities in different knowledge graphs (KGs). Current EA approaches suffer from scalability issues, limiting their usage in real-world EA scenarios. To tackle this challenge, we propose LargeEA to align entities between large-scale KGs. LargeEA consists of two channels, i.e., structure channel and name channel. For the structure channel, we present METIS-CPS, a memory-saving mini-batch generation strategy, to partition large KGs into smaller mini-batches. LargeEA, designed as a general tool, can adopt any existing EA approach to learn entities' structural features within each mini-batch independently. For the name channel, we first introduce NFF, a name feature fusion method, to capture rich name features of entities without involving any complex training process. Then, we exploit a name-based data augmentation to generate seed alignment without any human intervention. Such design fits common real-world scenarios much better, as seed alignment is not always available. Finally, LargeEA derives the EA results by fusing the structural features and name features of entities. Since no widely-acknowledged benchmark is available for large-scale EA evaluation, we also develop a large-scale EA benchmark called DBP1M extracted from real-world KGs. Extensive experiments confirm the superiority of LargeEA against state-of-the-art competitors.

==> preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

In this section, we first formalize the problem of entity alignment, and then present some background techniques.

\subsection{Problem Statement}
A knowledge graph (KG) can be denoted as $G = (E,R,T)$, where $E$ is the set of entities, $R$ is the set of relations, and $T=\{(h,r,t)~|~h,t \in E, r \in R\}$ \textcolor{red}{is the set of triples, each of which} represents the edge flowing from $h$ to $t$ via a relation $r$. 
Entity alignment (EA) \cite{OpenEA2020VLDB} aims to find the 1-to-1 mapping of entities $\psi$ from a source KG $G_s = (E_s,R_s,T_s)$ to a target KG $G_t = (E_t,R_t,T_t)$.
Formally, $\psi = \{(e_s, e_t) \in E_s \times E_t~|~e_s \equiv e_t\}$, where
$e_s \in E_s$, $e_t \in E_t$, and $\equiv$ means an equivalence relation between $e_s$ and $e_t$.
In most cases, a small set of equivalent entities $\psi^{\prime} \subset \psi$ is known beforehand and can be used as seed alignment (training data).
A representative experimental study \cite{OpenEA2020VLDB} has indicated that using a small set of seed alignment (e.g., 20\% of the total number of aligned entities) as training data conforms to the real-world.


\subsection{GNN-based EA Models}
Recently, graph neural networks (GNNs) have shown success in various domains. The core idea of GNNs is to learn each entity/vertex representation by capturing the information passing from its neighborhoods.
For the EA task, many GNN-based methods \cite{AttrGNN20,KECG19, EVA20, AliNet20} have present promising performances by propagating the alignment signal to the entity’s neighbors.
Therefore, we incorporate GNN-based models into the structure-based EA component in our \textsf{LargeEA} framework.
Generally, the GNN-based models align entities obeying the following equations \cite{RREA20}:
\begin{gather}%RREA
\boldsymbol{h}_{\mathcal{N}_{e_{i}}^{e}}^{l} \leftarrow \text{\emph{Aggregate}}\left(\left\{\boldsymbol{h}_{e_{k}}^{l}, \forall e_{k} \in\left\{e_{i}\right\} \cup \mathcal{N}_{e_{i}}^{e}\right\}\right)\\
\boldsymbol{h}_{e_{i}}^{l+1} \leftarrow \sigma\left(\boldsymbol{W}^{l} \cdot \boldsymbol{h}_{\mathcal{N}_{e_{i}}^{e}}^{l}\right)
\end{gather}
where $\boldsymbol{W}^{l}$ is the transformation matrix of layer $l$, $\boldsymbol{h}_{e_{k}}^{l}$ denotes the embedding of the entity $e_{k}^{l}$, and $\mathcal{N}_{e_{i}}^{e}$ represents the set of neighboring entities around $e_i$.
Eq. (1) is to aggregate information from the neighboring entities while Eq. (2) transforms the entity embeddings into better ones.
There are many operations available to serve the purpose of \emph{Aggregation}, such as normalized mean pooling (vanilla GCN~\cite{GCN17}) and attentional weighted summation (GAT~\cite{GAT18}).
